Densest Subgraphs of a Dense Erd\"os-R\'{e}nyi Graph. Asymptotics, Landscape and Universality

We consider the problem of estimating the edge density of densest $K$-node subgraphs of an Erd\"os-R\'{e}nyi graph $\mathbb{G}(n,1/2)$. The problem is well-understood in the regime $K=\Theta(\log n)$ and in the regime $K=\Theta(n)$. In the former case it can be reduced to the problem of estimating the size of largest cliques, and its extensions. In the latter case the full answer is known up to the order $n^{3\over 2}$ using sophisticated methods from the theory of spin glasses. The intermediate case $K=n^\alpha, \alpha\in (0,1)$ however is not well studied and this is our focus. We establish that that in this regime the density (that is the maximum number of edges supported by any $K$-node subgraph) is ${1\over 4}K^2+{1+o(1)\over 2}K^{3\over 2}\sqrt{\log (n/K)}$, w.h.p. as $n\to\infty$, and provide more refined asymptotics under the $o(\cdot)$, for various ranges of $\alpha$. This extends earlier similar results where this asymptotics was confirmed only when $\alpha$ is a small constant. We extend our results to the case of ''weighted'' graphs, when the weights have either Gaussian or arbitrary sub-Gaussian distributions. The proofs are based on the second moment method combined with concentration bounds, the Borell-TIS inequality for the Gaussian case and the Talagrand's inequality for the case of distributions with bounded support (including the $\mathbb{G}(n,1/2)$ case). The case of general distribution is treated using a novel symmetrized version of the Lindeberg argument, which reduces the general case to the Gaussian case. Finally, using the results above we conduct the landscape analysis of the related Hidden Clique Problem, and establish that it exhibits an overlap gap property when the size of the clique is $O(n^{2\over 3})$, confirming a hypothesis stated in a previous related work.

==> Introduction_old.tex <==

All order of magnitude notations $O(.), o(.), \omega(.), \Omega(.)$ should be understood with respect to $n$, that is the number of nodes in the graph. They are assumed
in the absolute sense, so that, for example, for a positive sequence $a_n>0$, $O(a_n)$ denotes any sequence $b_n$ with $\limsup_n|b_n|/a_n<\infty$.
Given sequences $a_n\ge 0, b_n>0, n\ge 1$ we write $a_n \lesssim b_n$ when $ \limsup_{n \to +\infty} \frac{a_n}{b_n} \leq 1$. $\gtrsim$ is defined similarly.
We write $a_n\sim b_n$ if $a_n\lesssim b_n$ and $a_n\gtrsim b_n$.

$\stackrel{d}{=}$ denotes equality in distribution. $|S|$ denotes the cardinality of a finite set $S$. Given a graph $G$ and a set of nodes
$S$ in it, we denote by $E[S]$ the set of edges spanned by $S$. 
We finish this section with some notational convention. $\mathcal{N}(\mu,\sigma^2)$ denotes the normal distribution with mean $\mu$ and
variance $\sigma^2$. $\Bern(p)$ denotes the Bernoulli distribution with parameter $p$. Namely $X=1$ with probability $p$ and $X=0$
with probability $1-p$ when $X\stackrel{d}{=} \Bern(p)$. $\mathcal{R}$ denotes the Rademacher distribution. Namely $X=\pm 1$ with
equal probability when $X\stackrel{d}{=} \mathcal{R}$. A random variable $X$ 
 has sub-Gaussian distribution if it has a strong tail decay, specifically if there are positive constants $a,b$ such that for all $t>0$ we have $\p(|X|>t)\leq a \exp(-bt^2)$. \dgedit{Define sub-Gaussian distribution. Make sure Gaussian is capitalized throughout the paper}

==> OGP_Gaussian.tex <==

\subsection{Gaussian Planted Clique Model}
\hedit{Fixing the Gaussian OGP computations is quite involved. The terms $Z_A$ have higher variance when they intersect the clique ($\binom{K}{2}$) than in the Bernoulli case ($\binom{K}{2}-\binom{z}{2}$), this implies (computationally) that the 1st moment bound $\Gamma$ is too small for the Gaussian setting, in particular since we look at $z = (1-\epsilon)K$. The natural way to deal with this would be to redefine a different fist moment bound $\Gamma$ for the Gaussian case then re-establish a result similar to Lemma 14.4, then proceed with computations for OGP proof. I will try to do this switch offline then update the below sections.} 

In the Gaussian setting of the planted clique problem, we first upper bound the the densest subgraphs using the first moment curve $\Gamma$.
\begin{proposition}\label{prop:1stmoment:ineq}
Let $1 \leq K =n^{\alpha}\leq n$ be integers with $\alpha \in (0, \frac{3}{2})$ and consider a random graph $G$ with a planted clique $\mathcal{PC}$ of size $K$ (as defined in Section \ref{Subsection 3.4} for general edge distributions). Then we have  for every $z\in \{\lfloor{\frac{K^2}{n}\rfloor}, \lfloor{\frac{K^2}{n}\rfloor}+1,...,K \} $ with high probability as $n \to +\infty$:
$$ \Psi_{K}^{\Nc\left(\frac{1}{2}, \frac{1}{4} \right)}(G)(z) \leq \Gamma_{K}(z) + o(K \log(K)).$$
\end{proposition}
\begin{proof}
 The case $K= z$ is straightforward, otherwise fix $z \in \{\lfloor{\frac{K^2}{n}\rfloor}, \lfloor{\frac{K^2}{n}\rfloor}+1,...,K-1 \} $.  Define then:
$$  Z_{\gamma, z} := \left|\left\{ A \subset V(G) : |A| = K, |A \cap \mathcal{PC}|=z, Z_A \geq \binom{z}{2}+\gamma \left(\binom{K}{2}- \binom{z}{2}   \right)  \right\} \right|.$$
where $Z_A$ is the sum of all edge random variables $Z_{i,j}$ with both vertices $i,j$ in $A$ and $V(A)$ is the set of vertices of graph $G$. Note that for each $A \subset V(G)$ with $|A|=K, |A\cap\mathcal{PC}|=z$, the density $Z_A$ follows a Gaussian distribution with mean $\frac{1}{2}\binom{z}{2}+\frac{1}{2}\binom{K}{2}$ and variance $\frac{1}{4}\binom{K}{2}$. Using first moment method we have:
\begin{align*}
  \p(Z_{\gamma, z} \geq 1) &\leq \E[Z_{\gamma, z} ]\\
  &= \E\left[   \sum_{ A \subset V(G) : |A| = K, |A \cap \mathcal{PC}|=z} \mathbf{1} \left( Z_A \geq \binom{z}{2} + \gamma \left(\binom{K}{2} - \binom{z}{2}\right)  \right) \right ] \\
  &= \binom{K}{z} \binom{n-K}{K - z} \p\left(  \mathcal{N}\left(\frac{1}{2} \left(\binom{K}{2} + \binom{z}{2}\right), \frac{1}{4}\left(\binom{K}{2} \right)\right) \geq  \binom{z}{2} + \gamma \left(\binom{K}{2} - \binom{z}{2}\right) \right)\\
&= \binom{K}{z} \binom{n-K}{K - z} \p\left(  \mathcal{N}(0,1)  \geq  2\left( \gamma-\frac{1}{2}\right) \frac{\binom{K}{2} - \binom{z}{2}}{ \sqrt{\binom{K}{2}}  } \right)\\ 
&\leq \binom{K}{z} \binom{n-K}{K - z}  \frac{1}{\sqrt{2\pi}} \frac{1}{  2( \gamma-\frac{1}{2}) \frac{\binom{K}{2} - \binom{z}{2}}{\sqrt{\binom{K}{2}}}} \exp\left( -2 \left( \gamma-\frac{1}{2}\right)^2 \left( \binom{K}{2} - \binom{z}{2} \right) \frac{\binom{K}{2} - \binom{z}{2}}{\binom{K}{2}}\right),
\end{align*}
taking the log, we show that for $\gamma := h^{-1}\left(\log 2 - \frac{\log( \binom{K}{z} \binom{n-K}{K-z}) }{\binom{K}{2} - \binom{z}{2}} \right) + \delta $  the first moment upper bound is $o(1)$, where $\delta := \left( \frac{\log( \binom{K}{z} \binom{n-K}{K-z}) }{\binom{K}{2} - \binom{z}{2}}  \right)^{\frac{5}{4}} $. Indeed, using Lemma \ref{Lemma 4.9} we have:
\begin{align*}
    \gamma &= \frac{1}{2} + \frac{1}{\sqrt{2}}\sqrt{\frac{\log( \binom{K}{z} \binom{n-K}{K-z}) }{\binom{K}{2} - \binom{z}{2}} } + O\left( \left(\frac{\log( \binom{K}{z} \binom{n-K}{K-z}) }{\binom{K}{2} - \binom{z}{2}}  \right)^{\frac{3}{2}}\right) + \delta,\\
\end{align*}
note that using elementary inequalities we have $\binom{K}{z} \leq K^{K-z} \leq n^{K-z}$ and $\binom{n-K}{K-z} \leq n^{K-z}$, therefore:
\begin{align*}
    \frac{\log( \binom{K}{z} \binom{n-K}{K-z}) }{\binom{K}{2} - \binom{z}{2}} &\leq \frac{2 (K-z)\log(n)}{\frac{(K-z)(K+z-1)}{2}}\\
    &= O\left(\frac{\log(K)}{K}\right),
\end{align*}
in particular, note that $\delta = \omega\left( \left(\frac{\log( \binom{K}{z} \binom{n-K}{K-z}) }{\binom{K}{2} - \binom{z}{2}} \right)^{\frac{3}{2}} \right)$ and $\delta = o\left( \frac{\log(K)}{K} \right)$. We have:
\begin{align*}
\hspace{-0.5cm}
2\left(\gamma - \frac{1}{2} \right)^2 \left( \binom{K}{2}-\binom{z}{2} \right) &= 2\left( \frac{1}{\sqrt{2}} \sqrt{\frac{\log( \binom{K}{z} \binom{n-K}{K-z}) }{\binom{K}{2} - \binom{z}{2}}  } + O\left(\frac{\log( \binom{K}{z} \binom{n-K}{K-z}) }{\binom{K}{2} - \binom{z}{2}}  \right)^{\frac{3}{2}} + \delta\right)^2 \left( \binom{K}{2} -\binom{z}{2} \right)\\
&=\log\left( \binom{K}{z} \binom{n-K}{K-z}\right) + 2\sqrt{2}\sqrt{\frac{\log( \binom{K}{z} \binom{n-K}{K-z}) }{\binom{K}{2} - \binom{z}{2}} } \left[  O\left(\frac{\log( \binom{K}{z} \binom{n-K}{K-z}) }{\binom{K}{2} - \binom{z}{2}}  \right)^{\frac{3}{2}} + \delta \right]\left( \binom{K}{2} -\binom{z}{2} \right)\\
&= \log\left( \binom{K}{z} \binom{n-K}{K-z}\right) + \Omega\left(\delta\sqrt{\frac{\log( \binom{K}{z} \binom{n-K}{K-z}) }{\binom{K}{2} - \binom{z}{2}} }  \left( \binom{K}{2} -\binom{z}{2} \right)  \right)\\
&= \log\left( \binom{K}{z} \binom{n-K}{K-z}\right) + \Omega\left( \delta \sqrt{\log\left( \binom{K}{z} \binom{n-K}{K-z}\right)  \left( \binom{K}{2} -\binom{z}{2} \right)} \right).
\end{align*}
Similarly:
\begin{align*}
    2\left(\gamma - \frac{1}{2} \right) \sqrt{\binom{K}{2}-\binom{z}{2}} &=\sqrt{\log\left( \binom{K}{z}\binom{n-K}{K-z}\right)} + o\left( \log\left( \binom{K}{z}\binom{n-K}{K-z}\right)\right)\\
    &\sim \sqrt{\log\left( \binom{K}{z}\binom{n-K}{K-z}\right)},
\end{align*}
we see then that:
\begin{align*}
\hspace{-1cm}
    &\binom{K}{z} \binom{n-K}{K - z}  \frac{1}{\sqrt{2\pi}} \frac{1}{2( \gamma-\frac{1}{2}) \sqrt{\binom{K}{2} - \binom{z}{2}}} \exp\left( -2 \left( \gamma-\frac{1}{2}\right)^2 \left( \binom{K}{2} - \binom{z}{2} \right)\right)\\
    &\sim  \binom{K}{z}\binom{n-K}{K-z} \frac{1}{\sqrt{2\pi} \sqrt{\log\left( \binom{K}{z}\binom{n-K}{K-z}\right)}}\exp \left( - \log\left( \binom{K}{z} \binom{n-K}{K-z}\right) - \Omega\left( \delta \sqrt{\log\left( \binom{K}{z} \binom{n-K}{K-z}\right)  \left( \binom{K}{2} -\binom{z}{2} \right)} \right)\right)\\
    &= \frac{1}{\sqrt{2\pi} \sqrt{\log\left( \binom{K}{z}\binom{n-K}{K-z}\right)}}\exp \left(  - \Omega\left( \delta \sqrt{\log\left( \binom{K}{z} \binom{n-K}{K-z}\right)  \left( \binom{K}{2} -\binom{z}{2} \right)} \right)\right)\\
    &= o(1).
\end{align*}
We have thus proven that with high probability as $n\to \infty$ :
\begin{align*}
    \Psi_{K}^{\Nc\left(\frac{1}{2}, \frac{1}{4} \right)}(G)(z) &\leq \binom{z}{2} + \gamma \left( \binom{K}{2} - \binom{z}{2}\right)\\
    &= \Gamma_{K}(z) + \delta \left( \binom{K}{2} -\binom{z}{2} \right)\\
    &= \Gamma_{K}(z) + o(K \log(K)),
 \end{align*}
 where we used in the last inequality $\delta = O\left( \left( \frac{\log(K)}{K} \right)^{\frac{5}{4}} \right) = o\left(\frac{\log(K)}{K}\right)$. 
\end{proof}
%In the case of Gaussian edge distribution, we assign values of $1$ to the edges of the Planted Clique and Gaussian r.v values to the remaining edges, this allows us to expand the definition of OGP in this setting by using the sum of edges as a measure of the density of any subgraph. 
In order to prove OGP in the Gaussian Planted Clique model we first need the following two Lemmas:
\begin{lemma}\label{Lemma 15.9}
Let $0 < m\leq K\leq n$ be positive integers and $G$ be a random graph with Planted Clique $\mathcal{PC}$ of size $K$. Define  $G_0 := G\setminus \mathcal{PC}$ the subgraph of $G$ obtained by removing $\mathcal{PC}$. Then:
$$ \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_K(G)(m) \geq \binom{m}{2} +\Psi^{\Nc\left(\frac{1}{2}, \frac{1}{4}\right)}_{m}(\mathcal{PC})+ \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_{K-m}(G_0) + \frac{(K-m)m}{2} - a(n) \sqrt{\frac{(K-m)m}{4}} ,$$
where $a(n)$ is any positive sequence s.t $a(n) \to_{n \to +\infty}=+\infty$.
\end{lemma}
\begin{proof}
 Fix $S_1$ to be the densest $m$-vertex subgraph of $\mathcal{PC}$ and let $N:= \binom{n-K}{K-m}$ be the number of different $K-m$ vertex subgraphs $S_2$ of $G_0$, optimizing over the choice of $S_2$ yields:
\begin{align*}
\Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_K(G)(m) &\geq \max_{S_2} |E(S_1 \cup S_2)|\\
&= \binom{m}{2}+\Psi^{\Nc\left(\frac{1}{2}, \frac{1}{4}\right)}_{m}(\mathcal{PC}) + \max_{S_2} \{ |E(S_1,S_2)| + |E(S_2)| \}. \numberthis \label{ineq:gaussian:ogp:lem:2}
 \end{align*} 
Where here $E(H)$ is the sum of all edge r.v over the subgraph $H$, in particular $E(S_2) \sim \mathcal{N}\left(\frac{1}{2}\binom{K-m}{2},\frac{1}{4}\binom{K-m}{2} \right)$ and $E(H,L)$ is the sum of all edge r.v between $H,L$ for $H\cap L = \emptyset$. Next, let's index the subsets $S_2$ by $S^i, i=1,...,N$ and set:
$$ Y_i = |E(S_1, S^i)|, X_i = |E(S^i)| ,$$
 note then that:
\begin{enumerate}
    \item $\forall i\in [N], X_i \sim \mathcal{N}\left(\frac{1}{2}\binom{K-m}{2},\frac{1}{4}\binom{K-m}{2} \right) .$
    \item $\forall i\in [N], Y_i \sim \mathcal{N} \left(  \frac{(K-m)m}{2}, \frac{(K-m)m}{4}\right) .$
    \item The sequence $X_i$ is independent from the sequence $Y_j$.
    \item $\max_{i \ [N]} X_i = \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_{K-m}(G_0).$
\end{enumerate}
We claim then that for any sequence $a(n)\to +\infty $ the following holds w.h.p as $n\to \infty$:
\begin{align*}
    \max_{i=1,...,N} \{X_i + Y_i\} &\geq \max_{i=1,...,N} X_i + \frac{(K-m)m}{2} - a(n)\sqrt{\frac{(K-m)m}{4}}. \numberthis \label{38.0}  
 \end{align*}
Indeed, let $i^* \in \arg \max X_i $, it suffices to prove that w.h.p:
$$ Y_{i^*} \geq  \frac{(K-m)m}{2} - a(n)\sqrt{\frac{(K-m)m}{4}}.$$
Since the sequences $X,Y$ are mutually independent, we see that $i^*$ is independent of the sequence $Y$, thus $Y_{i^*} \sim \mathcal{N} \left(  \frac{(K-m)m}{2}, \frac{(K-m)m}{4}\right)$. The claim then follows since $a(n) \to \infty$.
Combining \ref{ineq:gaussian:ogp:lem:2} with \ref{38.0} yields for any $a(n) =\omega_n(1)$:
\begin{align*}
\Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_K(G)(m) &\geq \binom{m}{2}+\Psi^{\Nc\left(\frac{1}{2}, \frac{1}{4}\right)}_{m}(\mathcal{PC}) + \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_{K-m}(G_0) + \frac{(K-m)m}{2} - a(n)\sqrt{\frac{(K-m)m}{4}},
\end{align*}
which ends the proof.
\end{proof}
\subsection{Proof of Theorem \ref{Theorem 3.14}}

\begin{proof}[Proof of Theorem \ref{Theorem 3.14}]
The proof proceeds as in the Bernoulli case, except that we do not need to make any further assumption in the regime $K = n^{\alpha}, \alpha\in [\frac{1}{2}, \frac{2}{3})$ as done in the Bernoulli case with Conjecture \ref{conjecture 3.3}. We first consider the regime $ \alpha\in (0, \frac{1}{2})$. We fix $\epsilon = \frac{1}{2}$, by Lemma \ref{Lemma 15.4}, there exists $C_0(\epsilon); C_1>0$ s.t 
$$ \max_{z \in I} \Gamma_K(z) + C_1 K\log(K) \leq \Gamma_K\left( \left\lfloor C_0 \frac{K^2}{n} \right\rfloor\right)  \leq \Gamma_K\left(\frac{K}{2}\right) ,$$
where $ I:= \mathbb{Z} \cap [D_1 \sqrt{K\log(K)}, D_2 \sqrt{K\log(K)}]$. Note in particular that since $K = o(\sqrt{n})$, we have $\lfloor{C_0 \frac{K^2}{n}}\rfloor=0$ for sufficiently large $n$. Hence, the previous inequality is equivalent to:
$$ \max_{z \in I} \Gamma_K(z) + C_1 K\log(K) \leq \Gamma_K(0) \leq \Gamma_K\left(\frac{K}{2}\right) .$$
Using Proposition \ref{prop:1stmoment:ineq},we see that in order to establish the presence OGP, it suffices to prove that:

$$  \min \left\{ \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_K(G)(0), \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_{K}(G)\left(\frac{K}{2}\right)\right\} \geq \Gamma_K(0) - o(K\log(K)).$$
The proof of $\Psi_K(G)(0) \geq \Gamma_K(0) - o(K\log(K)) $ is identical to the Bernoulli case (Section \ref{Subsection 15.2}) since we have by Theorem \ref{Theorem 3.6}:
$$ \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_K(G)(0) = \frac{1}{2} \binom{K}{2} + \frac{1}{2} V(n-K,K) + o\left(\sqrt{K}\log(K)\right) .$$
It remains then to prove that :
$$   \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_{K}(G)\left(\frac{K}{2}\right) \geq \Gamma_K(0) - o(K\log(K)).$$
We have by Lemma \ref{Lemma 15.9} (picking $a(n) := 4 \sqrt{\log(K)}$):
\begin{align*}
    \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_K(G)\left(\frac{K}{2}\right)   &\geq \binom{\frac{K}{2}}{2} +\Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_{\frac{K}{2}}(\mathcal{PC})+ \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_{\frac{K}{2}}(G_0) +\frac{K^2}{8}-  K\sqrt{\log(K)}
\end{align*}


Using Borell-Tis inequality, we have for $t>0$:
\begin{align*}
    \p\left(  \Psi^{\Nc\left(\frac{1}{2}, \frac{1}{4}\right)}_{m}(\mathcal{PC}) > \E\left[\Psi^{\Nc\left(\frac{1}{2}, \frac{1}{4}\right)}_{m}(\mathcal{PC}) \right] + t\right) \leq \exp\left(- C\frac{t^2}{m^2}\right)
\end{align*}
in particular, for $t=\frac{m^2}{4}$ and $m = \omega(1)$ we see that $\Psi^{\Nc\left(\frac{1}{2}, \frac{1}{4}\right)}_{m}(\mathcal{PC})  \geq \E\left[\Psi^{\Nc\left(\frac{1}{2}, \frac{1}{4}\right)}_{m}(\mathcal{PC}) \right] + \frac{m^2}{4}$ w.h.p. Note then that $\E\left[\Psi^{\Nc\left(\frac{1}{2}, \frac{1}{4}\right)}_{m}(\mathcal{PC}) \right] \gtrsim \frac{m^2}{4}$, we see then that the former inequality yields w.h.p:
$$  \Psi^{\Nc\left(\frac{1}{2}, \frac{1}{4}\right)}_{m}(\mathcal{PC})  \geq \frac{m^2}{4} $$
Therefore, we have w.h.p:

\begin{align*}
        \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_K(G)\left(\frac{K}{2}\right)   &\geq \binom{\frac{K}{2}}{2} +\frac{K^2}{16}+ \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_{\frac{K}{2}}(G_0) +\frac{K^2}{8}-  K\sqrt{\log(K)}\\
        &=\binom{\frac{K}{2}}{2} +\frac{K^2}{16}+ \frac{1}{2}\binom{\frac{K}{2}}{2} + \sqrt{ \frac{1}{2}  \binom{K}{2}\log\left(\binom{n-K}{\frac{K}{2}} \right )} +o(\sqrt{K} \log(K))  +\frac{K^2}{8}-  o(K \log(K)) \numberthis \label{50}\\
    &\sim \frac{6}{16}K^2,
\end{align*}

\newpage
Where \ref{50} follows from Theorem \ref{Theorem 3.6}. Moreover, we have know from previous computations in Section \ref{Subsection 15.2} in the Bernoulli case that $\Gamma_K(0)  \sim \frac{K^2}{4}$, thus we see that:
$$ \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_K(G)\left(\frac{K}{2}\right) - \Gamma_K(0) \gtrsim \frac{K^2}{4},$$
which yields the desired inequality $\Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_K(G)(\frac{K}{2}) \geq \Gamma_K(0) - o (K \log(K))$. This completes the proof of Theorem \ref{Theorem 3.14} when $ K =n^{\alpha} , \alpha \in (0, \frac{1}{2})$. We now deal with the case $\alpha \in [ \frac{1}{2}, \frac{2}{3})$, let $ m:= \lfloor C_0 \frac{K^2}{n} \rfloor$. We start by proving:
$$  \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_K(G)(m) \geq \Gamma_K(m) - o(K\log(K)).$$
We have by Lemma \ref{Lemma 15.9} (picking $a(n):= 2\sqrt{\log(K)}$) :
\begin{align*}
    \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_K(G)(m)   &\geq \binom{m}{2} +\Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_{m}(\mathcal{PC})+ \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_{K-m}(G_0) +\frac{1}{2}(K-m)m- \sqrt{(K-m)m \log(K)}.
    \end{align*}
Note then that using Theorems \ref{Theorem 3.6}, \ref{Theorem 3.8} we have that :
$$ \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_{K-m}(G_0) \geq U(n-K, K-m) - O(K \sqrt{\log(K) }) .$$
Recalling from $\ref{2}$ that $U(n,K) = V(n,K) \left(1 + O(\frac{1}{K})\right) = V(n,K) + O(\sqrt{K \log(K)})$ we see that :
$$ \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_{K-m}(G_0) \geq V(n-K, K-m) - O(K \sqrt{\log(K) }) .$$
Henceforth:
\begin{align*}
        \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_K(G)(m) &\geq  \binom{m}{2} + \frac{1}{2}\binom{K-m}{2} + \sqrt{ \frac{1}{2} \binom{K-m}{2}\log\left(\binom{n-K}{K-m}  \right)}+o(K \sqrt{\log(K)})   +\frac{(K-m)m}{2}   \\& -  \sqrt{(K-m)m \log(K)}  \\
    &= \binom{m}{2} + \frac{1}{2}\binom{K-m}{2} + \sqrt{ \frac{1}{2} \binom{K-m}{2}\log\left(\binom{n-K}{K-m} \right )}+o(K\log(K))   +\frac{(K-m)m}{2}  ,
\end{align*}
Further more, recall from \ref{43}:
\begin{align*}
    \Gamma_K(m) &= \frac{1}{2} \binom{m}{2} + \frac{1}{2} \binom{K}{2} + \frac{1}{\sqrt{2}} \sqrt{\left (\binom{K}{2} - \binom{m}{2}\right) \log\left(\binom{K}{m} \binom{n-K}{K-m}\right)  }   + o( K \log(K) ) .
\end{align*}
We are then in the exact same setting as in the Bernoulli computations in Section \ref{Subsection 15.2}, and thus :
$$  \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_K(G)(m) \geq \Gamma_K(m) - o(K\log(K)).$$
It remains then to prove that:
$$  \Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_K(G)\left(\frac{K}{2}\right) \geq \Gamma_K \left(m\right) - o(K\log(K)),$$
note then that using Theorems \ref{Theorem 3.6}, \ref{Theorem 3.8} the proof is identical to the regime $\alpha\in(0, \frac{1}{2})$ as one can show that $\Psi^{\Nc \left( \frac{1}{2}, \frac{1}{4}\right)}_K(G)\left(\frac{K}{2}\right) \gtrsim \frac{5}{16}K^2$ and $\Gamma_K \left(m\right) \sim \frac{K^2}{4}$. This then completes the proof of Theorem \ref{Theorem 3.14}.
\end{proof}

==> Proof_of_Upper_Bounds_in_Theorems_3.1,_3.2,_3.3.tex <==
Applying first moment inequality yields:
\begin{align*}
     \p\left(U_{\gamma_n} \geq 1\right) &\leq \E[U_{\gamma_n}] \\
     &= \binom{n}{K} \p\left( Z_S \geq \gamma_n \binom{K}{2}\right)\\
     & \leq \binom{n}{K} \theta \p\left(\mathcal{N}(0,1) \geq \gamma_n \sqrt{\binom{K}{2}} \right)\numberthis \label{13}\\
     &\leq \theta \binom{n}{K} \frac{1}{ \sqrt{2 \pi}\gamma_n \sqrt{\binom{K}{2}}} \exp\left( - \frac{\gamma_n^2 \binom{K}{2}}{2}\right) \numberthis \label{14}\\
    &\sim \theta \binom{n}{K} \frac{1}{ \sqrt{2 \pi} 2\sqrt{\frac{\log(\frac{n}{K})}{K}} \sqrt{\frac{K^2}{2}}} \exp\left( - \frac{\gamma_n^2 \binom{K}{2}}{2}\right) \numberthis \label{15}\\
     &= \frac{\theta}{2\sqrt{\pi}} \binom{n}{K} \frac{1}{\sqrt{K \log(\frac{n}{K})}} \exp\left( - \frac{\gamma_n^2 \binom{K}{2}}{2}\right),
\end{align*}
where we used Lemma \ref{Lemma 4.10} in (\ref{13}), standard Gaussian tail bound in $(\ref{14})$\footnote{Recall that for $x>0$ it holds $\p(\mathcal{N}(0,1) \geq x )\leq \frac{1}{x\sqrt{2\pi}} \exp\left(-\frac{x^2}{2}\right)$}, and replaced $\gamma_n$ by it's asymptotic equivalent in (\ref{15}). We see then that in order to have $U_{\gamma_n}=0$ w.h.p as $n\to +\infty$, it suffices to pick $\gamma_n $(i.e, pick $\delta_n$) such that $\binom{n}{K} \frac{1}{\sqrt{K \log(\frac{n}{K})}} \exp\left( - \frac{\gamma_n^2 \binom{K}{2}}{2}\right) = \epsilon_n$ where $ \epsilon_n$ is any positive sequence s.t $\epsilon_n  =o(1)$. Taking the log of the former yields:
$$ \binom{n}{K} \frac{1}{\sqrt{K \log(\frac{n}{K})}} \exp\left( - \frac{\gamma_n^2 \binom{K}{2}}{2}\right) = \epsilon_n \iff   \gamma_n = \sqrt{ \frac{2}{\binom{K}{2}}} \sqrt{       -\log(\epsilon_n)  + \log\left(   \binom{n}{K}\frac{1}{\sqrt{ K \log(\frac{n}{K})}}  \right)    } .$$
We choose $\epsilon_n$ s.t $ \log(\epsilon_n) = o\left( \log \left( \binom{n}{K} \frac{1}{\sqrt{K \log(\frac{n}{K})}} \right)\right)  = o\left( K \log(n) \right) $  where the second equality comes from part 3 of Lemma \ref{Lemma 4.5}. We then have: 

\begin{align*}
 &\gamma_n = \sqrt{ \frac{2}{\binom{K}{2}}}\sqrt{       -\log(\epsilon_n)  + \log\left(   \binom{n}{K}\frac{1}{\sqrt{ K \log(\frac{n}{K})}}  \right)    }  \\
 &\iff \gamma_n = \sqrt{ \frac{2}{\binom{K}{2}}} \sqrt{ \log\left(   \binom{n}{K}\frac{1}{\sqrt{ K \log(\frac{n}{K})}}  \right)   \left( 1 + \frac{-\log(\epsilon_n)}{\log\left( \binom{n}{K} \frac{1}{\sqrt{K \log(\frac{n}{K})}}\right)}\right) } \\
 &\iff \gamma_n = \sqrt{ \frac{2}{\binom{K}{2}}} \sqrt{ \log\left(   \binom{n}{K}\frac{1}{\sqrt{ K \log(\frac{n}{K})}}  \right) }   \left( 1 + O\left( \frac{-\log(\epsilon_n)}{\log\left( \binom{n}{K} \frac{1}{\sqrt{K \log(\frac{n}{K})}}\right)}\right) \right) \numberthis \label{16}\\
 &\iff \gamma_n = \sqrt{ \frac{2}{\binom{K}{2}}} \left(    \sqrt{      \log\left(   \binom{n}{K}\frac{1}{\sqrt{ K \log(\frac{n}{K})}}  \right)    }  + O\left( \frac{-\log(\epsilon_n)}{ \sqrt{      \log\left(   \binom{n}{K}\frac{1}{\sqrt{ K \log(\frac{n}{K})}}  \right)    }}\right)  \right)\\
    &\iff \gamma_n =   \sqrt{ \frac{2}{\binom{K}{2}}     \log\left(   \binom{n}{K}\frac{1}{\sqrt{ K \log(\frac{n}{K})}}  \right)    }  + O\left(\frac{-\log(\epsilon_n)}{K^{\frac{3}{2}}\sqrt{\log n}}\right), \\
\end{align*}
where \ref{16} follows from using the Taylor expansion of $\sqrt{1 + u}$ when $u\to 0$ with $u =\frac{-\log(\epsilon_n)}{\log\left( \binom{n}{K} \frac{1}{\sqrt{K \log(\frac{n}{K})}}\right)}=o(1) $. It remains to check that the above expression of $\gamma_n$ is consistent with its definition in terms of $\delta_n$. That is it suffices to prove that :
$$\sqrt{ \frac{2}{\binom{K}{2}}     \log\left(   \binom{n}{K}\frac{1}{\sqrt{ K \log(\frac{n}{K})}}  \right)    }  + O\left(\frac{-\log(\epsilon_n)}{K^{\frac{3}{2}}\sqrt{\log n}}\right) \sim 2 \sqrt{\frac{\log(\frac{n}{K})}{K}}.$$
We have by part 3 of Lemma \ref{Lemma 4.5}:
\begin{align*}
    \sqrt{ \frac{2}{\binom{K}{2}}     \log\left(   \binom{n}{K}\frac{1}{\sqrt{ K \log(\frac{n}{K})}}  \right)    } &= \sqrt{ \frac{2}{\binom{K}{2}}     \log\left(   \binom{n}{K}\right) -  \frac{2}{\binom{K}{2}}    \log\left(\sqrt{K \log\left(\frac{n}{K}\right)}\right)   }\\
    &\sim \sqrt{ \frac{2}{\frac{K^2}{2}} K \log\left( \frac{n}{K} \right) }\\
    &=2\sqrt{\frac{\log(\frac{n}{K})}{K}},
\end{align*}
and:
\begin{align*}
    O\left(\frac{-\log(\epsilon_n)}{K^{\frac{3}{2}}\sqrt{\log n}}\right) &= o\left( \frac{K \log(n)}{K^{\frac{3}{2}} \sqrt{\log(n)}} \right)\\
    &= o\left(\sqrt{\frac{\log(\frac{n}{K})}{K}}\right).
\end{align*}
Thus $\gamma_n \triangleq \sqrt{ \frac{2}{\binom{K}{2}}     \log\left(   \binom{n}{K}\frac{1}{\sqrt{ K \log(\frac{n}{K})}}  \right)    }  + O\left(\frac{-\log(\epsilon_n)}{K^{\frac{3}{2}}\sqrt{\log n}}\right) \sim 2 \sqrt{\frac{\log(\frac{n}{K})}{K}}$. We then have  w.h.p as $n\to +\infty$ that $U_{\gamma_n}=0$, equivalently:
\begin{align*}
\Psi^{\Rc}_{K}(G)  &\leq  \binom{K}{2} \left( \sqrt{ \frac{2}{\binom{K}{2}}     \log\left(   \binom{n}{K}\frac{1}{\sqrt{ K \log(\frac{n}{K})}}  \right)    }  + O\left(\frac{-\log(\epsilon_n)}{K^{\frac{3}{2}}\sqrt{\log(n)}}\right) \right)\\
&= \sqrt{2 \binom{K}{2} \log\left(   \binom{K}{n}\frac{1}{\sqrt{ K \log(\frac{n}{K})}}  \right)  } + O\left(-\log(\epsilon_n) \sqrt{\frac{K}{\log(n)}}\right).
\end{align*}


Recalling that $\epsilon_n$ was any sequence satisfying $\epsilon_n \to 0, \log(\epsilon_n) = o(K \log n)$, we obtain an upper bound:
$$\Psi^{\Rc}_{K}(G)  \leq \sqrt{2 \binom{K}{2} \log\left(   \binom{K}{n}\frac{1}{\sqrt{ K \log(\frac{n}{K})}}  \right)  } + O\left(a_n \sqrt{\frac{K}{\log(n)}}\right) ,$$
where $a_n$ is any sequence satisfying $a_n \to +\infty, a_n = o(K \log n)$. Furthermore, since this is an upper bound the condition $a_n = o(K \log n)$ can be dropped.


==> Proof_of_Upper_Bounds_in_Theorems_3.5,_3.6,_3.7.tex <==

We follow the same proof steps as in Section \ref{Proof of Upper Bounds in Theorems 3.1, 3.2, 3.4} to upper bound $\Psi^{\Nc}_K(G)$, and keep similar notations for $\gamma_n , U_{\gamma_n}$. Namely:
$$ U_{\gamma_n}  \triangleq \sum_{S \subset V(G), |S|=K,  Z_{i,j} \sim \mathcal{N}} \mathbf{1}\left(Z_S \geq \gamma_n \binom{K}{2}\right), $$
where $\gamma_n \traingleq (1 + \delta_n) 2\sqrt{\frac{\log \left( \frac{n}{K}\right)}{K}}$ and $\delta_n$ is some  sequence satisfying $\delta_n =o(1)$ that we will fix later. We have using standard Gaussian tail bounds
\begin{align*}
     \p\left(U_{\gamma_n} \geq 1\right) &\leq \E[U_{\gamma_n}] \\
    &= \binom{n}{K} \p\left( Z_S \geq \gamma_n \binom{K}{2}\right)\\
     &= \binom{n}{K} \p\left(\mathcal{N}(0,1) \geq \gamma_n \sqrt{\binom{K}{2}} \right)\\
     &\lesssim  \binom{n}{K} \frac{1}{ \sqrt{2\pi}\gamma_n \sqrt{\binom{K}{2}}} \exp\left( - \frac{\gamma_n^2 \binom{K}{2}}{2}\right)\\
     &\sim \frac{1}{2\sqrt{\pi}} \binom{n}{K} \frac{1}{\sqrt{K \log(\frac{n}{K})}} \exp\left( - \frac{\gamma_n^2 \binom{K}{2}}{2}\right).
\end{align*}
From here on we are in the same setting as in Section \ref{Proof of Upper Bounds in Theorems 3.1, 3.2, 3.4}, which then yields the same upper bound as in Theorem \ref{Theorem 3.1}.
